Analysis and Detectability of Offline Data Poisoning Attacks on Linear Dynamical Systems

In recent years, there has been a growing interest in the effects of data poisoning attacks on data-driven control methods. Poisoning attacks are well-known to the Machine Learning community, which, however, make use of assumptions, such as cross-sample independence, that in general do not hold for linear dynamical systems. Consequently, these systems require different attack and detection methods than those developed for supervised learning problems in the i.i.d.\ setting. Since most data-driven control algorithms make use of the least-squares estimator, we study how poisoning impacts the least-squares estimate through the lens of statistical testing, and question in what way data poisoning attacks can be detected. We establish under which conditions the set of models compatible with the data includes the true model of the system, and we analyze different poisoning strategies for the attacker. On the basis of the arguments hereby presented, we propose a stealthy data poisoning attack on the least-squares estimator that can escape classical statistical tests, and conclude by showing the efficiency of the proposed attack.

==> untargeted.tex <==
\subsection{Untargeted attacks}
Untargeted attacks aim at changing the perceived behaviour of the system, so that it is not possible to analyse the properties of the true system from the data.  We first focus  on attacks that only change the input signal, i.e. $\Delta X=0$. After that, we focus on attacks that only change the state measurement.



\subsubsection{Untargeted attacks on the input signal}
We are now concerned with untargeted attacks on the input signal, so $\Delta X=0$. For this particular case, we obtain the following result. 

\begin{lemma}\label{lemma:input_attack} Under an input attack $\Delta U_-$, if $\rank \begin{bmatrix}
    X_- \\ \tilde U_-
    \end{bmatrix}=m+n$, the LS estimates is $(A+\Delta A,B+\Delta B)$, where $(\Delta A,\Delta B)$ are
\begin{equation}\label{eq:solution_input_attack}
    \begin{bmatrix}
    \Delta A & \Delta B
    \end{bmatrix}  = -B\Delta U_- \begin{bmatrix}
    X_- \\ \tilde U_-
    \end{bmatrix}^\dagger.
\end{equation}
For this particular case, there exist a linear system that perfectly describes the data, i.e. $D=0$.
\end{lemma}
\begin{proof}
The LS estimate tries to find a solution for the following equation $
    X_+ = (A+\Delta A)X_- + (B+\Delta B)\tilde U_-.
$ Since also $X_+=AX_-+BU_-$ is satisfied, we conclude that
$
    \begin{bmatrix}
    \Delta A & \Delta B
    \end{bmatrix} \begin{bmatrix}
    X_- \\ \tilde U_-
    \end{bmatrix} = -B\Delta U_-
$. Using this last expression in \cref{eq:fundamental_eq_poisoned_system_simplified}, we conclude that $D=0$.
\end{proof}
Lemma \ref{lemma:input_attack} has a simple corollary, that any change $(\Delta A,\Delta B)$  in the true matrices of the system must belong to the image of $B$, i.e. $\begin{bmatrix}
    \Delta A & \Delta B
    \end{bmatrix} \in \image B$. Alternatively, if $\Delta U_- \in \ker B$, then $\begin{bmatrix}
    \Delta A & \Delta B
    \end{bmatrix}=0$.



\subsubsection{Untargeted attacks on the measured state signal}
We now turn our attention to attacks on the measured state signal. Similarly, as in the previous section, let $\Delta X = \begin{bmatrix}
\Delta x_0 & \dots & \Delta x_T
\end{bmatrix}$ be the poisoning signal, and define $\Delta X_- = \begin{bmatrix}
\Delta x_0 & \dots & \Delta x_{T-1}
\end{bmatrix}$, $\Delta X_+ = \begin{bmatrix}
\Delta x_1 & \dots & \Delta x_{T}
\end{bmatrix}$. Then, the poisoned data is $\tilde X_- = X_-+\Delta X_-$ (similarly for $\tilde X_+$).

\begin{lemma}
Under  a poisoning attack on the state signal $\Delta X$, the data is as if it was generated by a system  $(A+\Delta A_T,B+\Delta B_T)$, where $(\Delta A_T,\Delta B_T)$ are
\begin{equation}\label{eq:solution_state_attack}
    \begin{bmatrix}
    \Delta A_T & \Delta B_T
    \end{bmatrix}  = (\Delta X_+- A \Delta X_-) \begin{bmatrix}
    \tilde X_- \\ U_-
    \end{bmatrix}^\dagger.
\end{equation}
Consequently, if $\Delta X_+=A\Delta X_-$, then $\begin{bmatrix}
    \Delta A_T & \Delta B_T
    \end{bmatrix}=0$.
\end{lemma}
% \begin{proof}
% When $\Delta X$ is added to the measured state signals, it is equivalent to identifying the following system $
%     \tilde X_+ = (A+\Delta A)\tilde X_- + (B+\Delta B) U_-$.
% Subtracting $X_+=AX_-+BU_-$, we get
% $
% \Delta X_+= A \Delta X_- + \Delta A \tilde X_- +\Delta BU_-.
% $
% Consequently, the solution is given for
% $
% \begin{bmatrix}
% \Delta A & \Delta B
% \end{bmatrix} \begin{bmatrix}
% \tilde X_- \\ U_-
% \end{bmatrix} = \Delta X_+ - A\Delta X_-
% $, which conludes the proof.
% \end{proof}
The proof is omitted due to its similarity with that of lemma \ref{lemma:input_attack}. In contrast to lemma \ref{lemma:input_attack} we note 
that any non-zero change $(\Delta A,\Delta B)$ must belong to  $\image \left( ( \Delta X_+ - A\Delta X_-) \begin{bmatrix} \tilde X_-^\top & U_-^\top\end{bmatrix}\right)$.


Differently from the previous case, we must distinguish between \textit{oblivious} and \textit{adaptive} adversaries. For an oblivious adversary we can derive a result similar to that in lemma \ref{lemma:input_attack_indistinguishable_asymptotics}.
\begin{lemma}\label{lemma:state_attack_asymptotics}
Let $\Delta\theta_T=(\Delta A_T,\Delta B_T)$ be the solution of \cref{eq:solution_state_attack}, and assume that $\Delta x_t=-x_t+a_t$, where $a_t$ is uncorrelated from $x_t$ and follows the same distribution as $u_t$. Then, $(u_t,\tilde u_t)$ are indistinguishable, and, if $A$ is stable, $\theta_T$ converges to
\begin{equation}\lim_{T\to\infty} \Delta\theta_T = (0,-B)\end{equation}
\end{lemma}
